Developmentally motivated emergence of compositional communication via template transfer

This paper explores a novel approach to achieving emergent compositional communication in multi-agent systems. We propose a training regime implementing template transfer, the idea of carrying over learned biases across contexts. In our method, a sender-receiver pair is first trained with disentangled loss functions and then the receiver is transferred to train a new sender with a standard loss. Unlike other methods (e.g. the obverter algorithm), our approach does not require imposing inductive biases on the architecture of the agents. We experimentally show the emergence of compositional communication using topographical similarity, zero-shot generalization and context independence as evaluation metrics. The presented approach is connected to an important line of work in semiotics and developmental psycholinguistics: it supports a conjecture that compositional communication is scaffolded on simpler communication protocols.

==> Old/removed_by_pm.tex <==
\paragraph{Object naming game}
 We focus on a Lewis signaling game \citep{lewis_convention:_2011,skyrms_signals:_2010} called \textit{object naming game}: two agents, a sender and a receiver, learn to communicate about colored geometric objects. The sender observes an object (an image represented as an array), sends a message (a sequence of discrete symbols) to the receiver, and the receiver must correctly predict both the color and the shape of the object. The agents are rewarded when the receiver correctly predicts the shape and the color of the object seen by sender. \ppm{The agents are rewarded ..., seems to me uninformative} More formally, the agents are optimized to maximize the log likelihood of both color and shape given the receiver's predictions as described by:
 
\begin{equation}
\label{loss}
    \mathcal{L} = \mathbb{E}_{\substack{x, y_c, y_s}} \mathbb{E}_{m \sim s(m \vert x)} [-\log r(y_c, y_s \vert m)],
\end{equation}

where $s$ is the policy of the sender (i.e. $s(m|x)$ is the probability of sending the message $m$ when observing image $x$), $r$ is the policy of the receiver, $x$ is the representation of the object and $y_c, y_s$ are ground truth labels for the color and shape. \ppm{There are number of issues with the formula. 1. I'd prefer to make parameters explicit. 2. If they stay implicit we need to state that polices are parametrized/learnable. 3. It seems to me that we do not need $x$. 4. Generally, less is better, do not use $\hat{\cdot}$ unless it is useful.}

\paragraph{Pre-training games}
Let us consider an extension of the above signaling game. Before the actual game is played, there is a pre-training phase in which two senders ($s_1, s_2$) take turns communicating with one receiver and playing two separate games: color naming game and shape naming game (as described by \eqref{pretraining-loss-1} and \eqref{pretraining-loss-2}). Each of the senders is optimized to maximize accurate predictions of only one aspect of the object, color or shape, respectively. This can be seen as alternating between these two losses\ppm{"alternating" is a strange word here.}:
\begin{equation}
\label{pretraining-loss-1}
    \mathcal{L}_1 = \mathbb{E}_{\substack{x, y_c}} \mathbb{E}_{m \sim s_1(m_1 \vert x)} [-\log r(y_c \vert m_1)]
\end{equation}
\begin{equation}
\label{pretraining-loss-2}
    \mathcal{L}_2= \mathbb{E}_{\substack{x, y_s}} \mathbb{E}_{m \sim s_2(m_2 \vert x)} [-\log r(y_s, \vert m_2)]
\end{equation}
The loss of the pre-training game is disentangled in the sense that each of two senders is incentivized to specialize in communicating either shape, or color
\ppm{The loss of the pre-training... I can see little knowledge in this sentence. We may keep the word "disentangled" somewhere}. After pre-training ends (the stopping criterion is an accuracy threshold), the receiver is passed over (a procedure we call \textit{template transfer}) to the object naming game (as described in the previous paragraph) with a new sender $s$. To minimize its loss, the new sender $s$ must then learn receiver $r$'s pre-trained communication protocol, i.e. its messages must resemble messages sent by two specialized senders $s_1$ and $s_2$ from the pre-training game. This turns out to be a sufficient incentive for compositionality to emerge. (See Figure \ref{fig:procedure} for a depiction of the whole procedure.) \ppm{This section needs better marketing. It is the main result, the novelty etc ;)}

\begin{figure}[h]
\centering
\includegraphics[width=0.5\linewidth]{img/template_transfer(1).png}
\caption{Template transfer consists of pre-traning the receiver $r$ on a two games with disentangled losses $\mathcal{L}_1$ and $\mathcal{L}_2$ and transferring it to a new object naming game. }
\label{fig:procedure}
\end{figure}
\ppm{On the figure the loss is $L$ and $\mathcal{L}$ otherwise.}


\paragraph{Measuring compositionality}
We utilize three metrics of compositionality of a communication protocol: \textit{zero-shot generalization accuracy, context independence and topographical similarity.} To measure the capacity for zero-shot generalization, we first split the dataset into training set and test set, so that the latter contains previously unseen pairs of previously seen shapes and colors. The agents are trained on the training set and evaluated on the test set (with sender's softmax replaced with argmax to ensure deterministic language).


Context independence was introduced by \cite{bogin_emergence_2018} as a measure of alignment between agent’s symbols $s$ out of which messages are composed and task concepts $c$ (in our case, shape and color). Let $v^c = \argmax_v p(c \vert v)$. Then, context independence is defined as $\mathbb{E}_c ( p(v^c \vert c) \cdot p(c \vert v^c))$. Note that context independence can be seen as an overly restrictive metric as it punishes the formation of synonyms \citep{lowe_pitfalls_2019}.

Finally, topographical similarity \citep{brighton_understanding_2006,lazaridou_emergence_2018}, also known as Representational Similarity Analysis \citep{kriegeskorte_representational_2008,bouchacourt_how_2018}, measures the correlation between the structure of targets ($y_c$ and $y_s$) and the structure of messages ($m$). We first compute Levenshtein distance between each pair of targets and each pair of messages, obtaining two symmetric distance matrices. Then we compute the Spearman $\rho$ correlation coefficient between upper triangular parts of both of these distance matrices.
